A Self-Organizing Tensor Architecture for Multi-View Clustering

In many real-world applications, data are often unlabeled and comprised of different representations/views which often provide information complementary to each other. Although several multi-view clustering methods have been proposed, most of them routinely assume one weight for one view of features, and thus inter-view correlations are only considered at the view-level. These approaches, however, fail to explore the explicit correlations between features across multiple views. In this paper, we introduce a tensor-based approach to incorporate the higher-order interactions among multiple views as a tensor structure. Specifically, we propose a multi-linear multi-view clustering (MMC) method that can efficiently explore the full-order structural information among all views and reveal the underlying subspace structure embedded within the tensor. Extensive experiments on real-world datasets demonstrate that our proposed MMC algorithm clearly outperforms other related state-of-the-art methods.

==> table_notation.tex <==
\begin{table}
\small
\centering
\caption{List of basic symbols.}
\label{tab:notation}
\footnotesize
\begin{tabular}{ll}
\toprule
Symbol & Definition and description\\
\midrule
$x$ & lowercase letter represents scale\\
$\mathbf{x}$ & boldface lowercase letter represents vector\\
$\mathbf{X}$ & boldface uppercase letter represents matrix\\
$\mathcal{X}$ & calligraphic letter represents tensor\\
$[1:M]$ & a set of integers in the range of $1$ to $M$ inclusively \\
$\left\langle\cdot,\cdot\right\rangle$ & denotes inner product\\
$\circ$ & denotes outer product\\
$\ast$ & denotes Hadamard (elementwise) product\\
$\otimes$ & denotes Kronecker product\\
 $\mathbf{A}_\mathbf{B}$ & denotes $\mathbf{A} \otimes \mathbf{B}$ \\
$tr(\cdot)$   & denotes trace function \\
$diag(\cdot)$ & denotes a diagonal matrix \\
$vec(\cdot)$  & denotes the column stacking operator \\
$\left\|\cdot\right\|_{F}$ & denotes Frobenius norm of matrix or tensor\\
$\left\|\cdot\right\|_{2,1}$ & denotes $\ell_{2,1}$ norm of matrix\\
\bottomrule
\end{tabular}
\vspace{-5pt}
\end{table}
% $\left|\cdot\right|$ & denotes absolute value\\



% \begin{table}
% \small
% \caption{Symbols.}
% \label{tab:notation}
% \begin{tabular}{ll}
% \toprule
% Symbol & Definition and description\\
% \midrule
% $x$ & each lowercase letter represents a scale\\
% $\mathbf{x}$ & each boldface lowercase letter represents a vector\\
% $\mathbf{X}$ & each boldface capital letter represents a matrix\\
% $\mathcal{X}$ & each calligraphic letter represents a tensor, set or space\\
% $[1:M]$ & a set of integers in the range of $1$ to $M$ inclusively. \\
% $\left\langle\cdot,\cdot\right\rangle$ & denotes inner product\\
% $\circ$ & denotes outer product\\
% $\ast$ & denotes Hadamard (elementwise) product\\
% $\left|\cdot\right|$ & denotes absolute value\\
% $\left\|\cdot\right\|_{F}$ & denotes (Frobenius) norm of vector, matrix or tensor\\
% $\left\|\cdot\right\|_{2,1}$ & denotes $\ell_{2,1}$ norm of the given matrix\\
% \bottomrule
% \end{tabular}
% \end{table}
